Graph Quasirandomness for Hypothesis Testing of Stochastic Block Models

The celebrated theorem of Chung, Graham, and Wilson on quasirandom graphs implies that if the 4-cycle and edge counts in a graph $G$ are both close to their typical number in $\mathbb{G}(n,1/2),$ then this also holds for the counts of subgraphs isomorphic to $H$ for any $H$ of constant size. We aim to prove a similar statement where the notion of close is whether the given (signed) subgraph count can be used as a test between $\mathbb{G}(n,1/2)$ and a stochastic block model $\mathbb{SBM}.$ Quantitatively, this is related to approximately maximizing $H \longrightarrow |\Phi(H)|^{\frac{1}{|\mathsf{V}(H)|}},$ where $\Phi(H)$ is the Fourier coefficient of $\mathbb{SBM}$, indexed by subgraph $H.$ This formulation turns out to be equivalent to approximately maximizing the partition function of a spin model over alphabet equal to the community labels in $\mathbb{SBM}.$ We resolve the approximate maximization when $\mathbb{SBM}$ satisfies one of four conditions: 1) the probability of an edge between any two vertices in different communities is exactly $1/2$; 2) the probability of an edge between two vertices from any two communities is at least $1/2$ (this case is also covered in a recent work of Yu, Zadik, and Zhang); 3) the probability of belonging to any given community is at least $c$ for some universal constant $c>0$; 4) $\mathbb{SBM}$ has two communities. In each of these cases, we show that there is an approximate maximizer of $|\Phi(H)|^{\frac{1}{|\mathsf{V}(H)|}}$ in the set $\mathsf{A} = \{\text{stars, 4-cycle}\}.$ This implies that if there exists a constant-degree polynomial test distinguishing $\mathbb{G}(n,1/2)$ and $\mathbb{SBM},$ then the two distributions can also be distinguished via the signed count of some graph in $\mathsf{A}.$ We conjecture that the same holds true for distinguishing $\mathbb{G}(n,1/2)$ and any graphon if we also add triangles to $\mathsf{A}.$

==> 2SBM.tex <==
\section{2-SBM}

==> RstrictedModels.tex <==
\section{Restricted Stochastic Block Models}
Since stochastic block models capture all probabilistic latent space models, it is worthwhile studying the scaled Fourier coefficients for specific stochastic block models. We begin with two very simple cases.

\subsection{``Non-Negative'' Stochastic Block Models}
\label{sec:nonnegative}
\begin{theorem} Consider an instance $\sbm(n,P, \distribution)$ for some matrix $P$ such that $P_{ij}\ge 1/2$ for each $i,j.$ Then, for any subgraph $H,$ it holds that 
$$
|\ESW_{\sbm(n,P,\distribution)}(H)|^{1/|V(H)|}\le
\max_{t\le |V(H)|-1}
|\ESW_{\sbm(n,P,\distribution)}(\Star_t)|^{1/(t+1)}.
$$
\end{theorem}
\begin{proof}
Let $P\in [0,1]^{r\times r}$ and $P_{i,j}= 1/2 + \psi_{i,j},$ where $\psi_{i,j}\ge0$ for each $i,j.$ Let $q_i = \prob_{X\sim\distribution}[X=i].$
Then, for any graph $H$ on vertex set $[h],$
$$
|\ESW_{\sbm(n,P,\distribution)}(H)| = 
\ESW_{\sbm(n,P,\distribution)}(H)= 
\sum_{x_1, x_2,\ldots,x_h\in [r]^h}
\prod_{s=1}^h 
q_{x_s}
\times
\prod_{(ij)\in E(H)}
2\psi_{x_ix_j}.
$$
In particular, this clearly shows that $\ESW_{\sbm(n,P,\distribution)}(H)$ is strictly decreasing under removing edges. Hence, for any fixed number of non-isolated vertices $h,$ $|\ESW_{\sbm(n,P\distribution)}(H)|^{1/|V(H)|}$ is maximized when it is a union of disjoint stars. Using \cref{eq:disjointunions}, this immediately gives the desired conclusion.\end{proof}

It turns out that a simple construction of a non-negative stochastic block model with two communities shows that arbitrarily large stars are needed.

\begin{proposition}[\color{red}In progress]
Consider a 2-community stochastic block model with\linebreak  $P = \begin{pmatrix}
 \frac{1}{2} \; & \frac{1}{2} + n^{-(\frac{1}{2}+\alpha)}\\
\frac{1}{2} + n^{-(\frac{1}{2}+\alpha)}\; &\frac{1}{2}
\end{pmatrix}$ and $\distribution$ given by $q_1 = n^{-(\frac{1}{2}-t\alpha)}, q_2 = 1-q_1.$ Then, ...
\end{proposition}
\begin{proof}
Consider any connected graph $H.$ Then, 
$$
\ESW_{\sbm(n,P,\distribution)}(H)= 
\sum_{S\subseteq V(H)}
q_1^{|S|}
q_2^{|V(H)| -|S|}
0^{|E(H)|_{S\times S}|}
(n^{-(\frac{1}{2}+\alpha)})^{|E(H)|_{(V(H)\backslash S)\times S}|}
0^{|E(H)|_{(V(H)\backslash S)\times(V(H)\backslash S)}|}.
$$
In particular, this means that if $H$ is not bipartite, the expression is 0 and if $H$ has parts of sizes $h_1\le  h_2,$ 
$$
\ESW_{\sbm(n,P,\distribution)}(H)= 
n^{-\alpha |E(H)|}
\Bigg((q_1)^{h_1}
(q_2)^{h_2} + 
(q_1)^{h_2}
(q_2)^{h_1}
\Bigg) = 
\Theta(n^{-(\frac{1}{2}+\alpha)|E(H)|} n^{-h_1(\frac{1}{2} - t\alpha)}).
$$
In particular, this means that for any fixed $h_1,h_2,$ the above expression is maximized whenever $H$ is as as sparse as possible without having isolated vertices, i.e. it is a union of stars. Using \cref{eq:disjointunions}, we can assume that it is a star. In fact, it clearly follows that for any $H$ that is not a star, for the star on the same number of vertices
$$
|\ESW_{\sbm(n,P,\distribution)}(H)|^{1/|V(H)|} = 
o\Bigg(|\ESW_{\sbm(n,P,\distribution)}(\Star_{|V(H)|-1})|^{1/|V(H)|}\Bigg).
$$
Now, suppose that $H = \Star_{r}.$ Then, 
\begin{align*}
    & |\ESW_{\sbm(n,P,\distribution)}(H)|^{1/|V(H)|}\\
    & = 
   \Theta(n^{-(\frac{1}{2}+\alpha)r} n^{-(\frac{1}{2} - t\alpha)})^{1/(r+1)} = 
   \Theta(n^{-1/2})\times 
   \Theta(n^{-\frac{\alpha(t-r)}{r+1}}).
\end{align*}
By taking $\alpha$ a small positive value, we conclude that 
$$
|\ESW_{\sbm(n,P,\distribution)}(\Star_r)|^{1/(r+1)} = \omega(|\ESW_{\sbm(n,P,\distribution)}(\Star_y)|^{1/(y+1)})\; \; \forall y < t.
$$
Taking $\alpha$ a small negative value, we conclude that
$$
|\ESW_{\sbm(n,P,\distribution)}(\Star_r)|^{1/(r+1)} = \omega(|\ESW_{\sbm(n,P,\distribution)}(\Star_y)|^{1/(y+1)})\; \; \forall y > t.
$$

\end{proof}




\subsection{Diagonal Stochastic Block Models}
\begin{theorem} Consider an instance $\sbm(n,P, \distribution)$ for some matrix $P$ such that $P_{ij}= 1/2$ whenever $i\neq j.$ Then, for any subgraph $H,$ it holds that 
\begin{align*}
& |\ESW_{\sbm(n,P,\distribution)}(H)|^{1/|V(H)|}\\
& \le
\max\Bigg(
|\ESW_{\sbm(n,P,\distribution)}(\Star_1)|^{1/2},
|\ESW_{\sbm(n,P,\distribution)}(\Star_2)|^{1/3},
|\ESW_{\sbm(n,P,\distribution)}(C_4)|^{1/4}
\Bigg).
\end{align*}
\end{theorem}
\begin{proof}
It is enough to consider the case when $H$ is connected. Let $|V(H)|= h$ and $P_{ii}= 1/2+\psi_{ii}$ for all $1\le i \le r.$
Let $q_i = \prob_{X\sim\distribution}[X=i].$
Then, one can trivially show that 
$$
\ESW_{\sbm(n,P,\distribution)}(H) = 
\sum_{i=1}^r q^h_i(2\psi_{ii})^{|E(H)|}.
$$
\paragraph{Case 1)} If $|V(H)|$ is odd or $|E(H)|=h-1\ge 2,$ 
$$
|\ESW_{\sbm(n,P,\distribution)}(H)|\le
|\sum_{i=1}^r q^h_i(2\psi_{ii})^{|V(H)|-1}|\le 
\sum_{i=1}^r q^h_i|2\psi_{ii}|^{|V(H)|}\times\frac{1}{|2\psi_{ii}|}.
$$
Now, using the fact that $|2\psi_{ii}|\le 1$ and inequality between $L_p$-norms, we conclude that 
$$
\Bigg(
\sum_{i=1}^r q^h_i|2\psi_{ii}|^{|V(H)|}\times\frac{1}{|2\psi_{ii}|}
\Bigg)^{1/h}\le 
\Bigg(
\sum_{i=1}^r q^3_i|2\psi_{ii}|^{3}\times\frac{1}{|2\psi_{ii}|}
\Bigg)^{1/3}= 
|\ESW_{\sbm(n,P,\distribution)}(\Star_2)|^{1/3}.
$$
\paragraph{Case 2)} If $|V(H)|$ is even and 
$|E(H)|\ge |V(H)|\ge 4,$
, 
$$
|\ESW_{\sbm(n,P,\distribution)}(H)|^{1/|V(H)|}\le
\Bigg(\sum_{i=1} q^h_i(2\psi_{ii})^{h}\Bigg)^{1/h}\le  
\Bigg(\sum_{i=1} q^4_i(2\psi_{ii})^{4}\Bigg)^{1/4} = 
|\ESW_{\sbm(n,P,\distribution)}(C_4)|^{1/|V(4)|}
$$

\end{proof}
\subsection{Stochastic Block Models with 2 Communities}
Now that we have addressed the easy block-diagonal and positive cases, we attempt to tackle the general case. For simplicity, we begin with two communities. That is $P =\begin{pmatrix}1/2+ \psi_{1,1}\; 1/2 +\psi_{1,2}\\
1/2 + \psi_{1,2}\; 1/2 +\psi_{2,2}
\end{pmatrix}$ and $\distribution = (q,1-q).$ To avoid the previous two cases, we assume that $\psi_{1,2}\neq 0$ and $\psi_{1,1},\psi_{1,2}, \psi_{2,2}$ do not all have the same sign. 

First, for any graph $H,$ we have 
\begin{equation}
\label{eq:2sbmsignedweight}
    \begin{split}
        & \ESW_{\sbm(n,P,\distribution)}(H)\\
        & =\sum_{S\subseteq V(H)}
        q^{|S|}(1-q)^{|V(H)|-|S|}
        (2\psi_{11})^{|E(H)_{S\times S}|}
        (2\psi_{12})^{|E(H)_{S\times (V(H)\backslash S)}|}
        (2\psi_{22})^{|E(H)_{(V(H)\backslash S)\times (V(H)\backslash S)}|}.
    \end{split}
\end{equation}
\subsubsection{The Independence Polynomial Interpretation}
Now, we specialize to the case when $\psi_{1,1}= 0.$
Then, $\psi_{1,2}\psi_{2,2}<0$ as we are otherwise in the all positive (all negative) model. 
Note that unless $S$ is an independent set, the summand becomes equal to 0. Hence, the expression in  \cref{eq:2sbmsignedweight} becomes 
\begin{equation}
\label{eq:independencepolynomial}
    \begin{split}
        & \sum_{S\in \mathcal{I}(H)}
        q^{|S|}(1-q)^{|V(H)|-|S|}
        (2\psi_{12})^{|E(H)_{S\times (V(H)\backslash S)}|}
        (2\psi_{22})^{|E(H)_{(V(H)\backslash S)\times (V(H)\backslash S)}}\\
        & =(1-q)^{|V(H)|}
        (2\psi_{2,2})^{|E(H)|}
        \sum_{S\in \mathcal{I}(H)}
        \Bigg(\frac{q}{1-q}\Bigg)^{|S|}
        \Bigg(\frac{\psi_{1,2}}{\psi_{2,2}}\Bigg)^
        {|E(H)_{S\times (V(H)\backslash S)}|}\\
        & =
        (1-q)^{|V(H)|}
        (2\psi_{2,2})^{|E(H)|}
        \sum_{S\in \mathcal{I}(H)}
        \prod_{i\in S}
        \Big(\frac{q}{1-q}\Big)\times 
        \Bigg(\frac{\psi_{1,2}}{\psi_{2,2}}\Bigg)^
        {\deg_H(i)}\\
        & =
        (1-q)^{|V(H)|}
        (2\psi_{2,2})^{|E(H)|}\times 
        Z_H\Bigg(
        \frac{q}{1-q}\Bigg(\frac{\psi_{1,2}}{\psi_{2,2}}\Bigg)^
        {\deg_H(1)},
        \frac{q}{1-q}\Bigg(\frac{\psi_{1,2}}{\psi_{2,2}}\Bigg)^
        {\deg_H(2)},
        \ldots,
        \frac{q}{1-q}\Bigg(\frac{\psi_{1,2}}{\psi_{2,2}}\Bigg)^
        {\deg_H(h)}
        \Bigg).
    \end{split}
\end{equation}
where $Z_H$ is the independence polynomial of $H.$

Thus, in trying to optimize the above expression over $H,$ one could first optimize the value of $Z_H$ (with respect to the specific input) over all graphs on $h =|V(H)|$ vertices and $e= |E(H)|$ and then optimize (raising to the power $1/h$) over $v,h.$

The problem of maximizing the independence polynomial subject to vertex and edge constraints has a long history in the combinatorics and statistical physics literature. Of special interest is also the scaling $Z_H(\lambda)^{1/|V(H)|}$ due to its relevance to bounding the number of independent sets. 

To the best of our knowledge, the state-of-the-art for graphs of irregular degrees is \cite{Sah_2019}. What makes \cref{eq:independencepolynomial} qualitatively very different from previous work is that in the ``interesting regime'' one needs to optimize when the input variables $\displaystyle \frac{q}{1-q}\Bigg(\frac{\psi_{1,2}}{\psi_{2,2}}\Bigg)^{\deg_H(i)}$ are potentially negative. This seems to have very non-trivial implications as some of the main arguments used in the literature such as the bipartite swapping trick of \cite{ZHAO_2009} and natural probabilistic interpretations (in terms of the corresponding hardcore model) do not immediately carry over. 

\begin{remark} If one does not impose $\psi_{1,1}=0,$ the problem is similarly related to optimizing the partition function of a 2-spin model over graphs with a fixed number of vertices and edges. In general, in the case of $r\ge 2$ communities, one needs to optimize the partition function of an $r$-spin model.  
\end{remark}

==> SomeSimpleCases.tex <==
\section{Several Simple Models}
\subsection{Non-Negative Models}
\subsection{Diagonal Models}

==> full2SBM.tex <==
\section{Full Analysis of the 2-SBM Case}
Parametrize the 2-SBM by 
$\Omega = \{1,2\},\mathcal{D} = (p,1-p),\sigma(i,j) = (1  + \beta_{i,j})/2.$ Call this model $\SBM(p,1-p, \beta)$ where $\beta = (\beta_{11}, \beta_{12}, \beta_{22}).$ WLOG, assume that $p\le 1-p.$
\begin{theorem}
\label{thm:2sbmtheorem}
For any connected subgraph $H,$
\begin{equation}
\label{eq:comparisonin2sbm}
    \begin{split}
        & |\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}\\
        & \le C(H)\times 
        \max \Big\{|\ESW_{\SBM(p,1-p, \beta)}(K)|^{1/|V(K)|}\; : \; K \text{ is a 4-cycle or a star with at most $|V(H)|+1$ vertices}\Big\}
    \end{split}
\end{equation}
for some constant $C(H)$ depending \emph{only} on $H,$ but crucially not on $\SBM(p,1-p, \beta).$
\end{theorem}

\paragraph{High-level idea.}
The main idea of the proof is the following. Take any subgraph $H$ and suppose for the sake of contradiction that \cref{eq:comparisonin2sbm} does not hold for some large $C(H).$ Hence, in particular,
$$
|\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}\ge C(H) \times\max_{1\le t \le D} |\ESW_{\SBM(p,1-p, \beta)}(\Star_t)|^{1/(t+1)}.
$$

Clearly, $|\ESW_{\SBM(p,1-p, \beta)}(H)|\le |\ESW_{\SBM(p,1-p, |\beta|)}(H)|$ where $|\beta| = (|\beta_{11}|, |\beta_{12}|, |\beta_{22}|).$ On the other hand, since $\SBM(p,1-p, |\beta|)$ is a non-negative model, by \cref{sec:nonnegative}\linebreak  $|\ESW_{\SBM(p,1-p, |\beta|)}(H)|^{1/|V(H)|}\le 
|\ESW_{\SBM(p,1-p, |\beta|)}(\Star_t)|^{1/(t+1)}
$ for some $t\in {1,2,\ldots, |V(H)|-1}.$ Thus, 
\begin{equation}
\label{eq:starandHwithmodulus}
\begin{split}
& |\ESW_{\SBM(p,1-p, |\beta|)}(\Star_t)|^{1/(t+1)}\ge 
|\ESW_{\SBM(p,1-p, |\beta|)}(H)|^{1/|V(H)|}\\
& \ge 
|\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}\ge 
C(H)|\ESW_{\SBM(p,1-p, \beta)}(\Star_t)|^{1/(t+1)}.
\end{split}
\end{equation}
Explicitly writing the expectations of $t$-stars out, we conclude that 
\begin{equation}
\label{eq:starfailureequation}
\begin{split}
&\Bigg|
p(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|)^t + 
(1-p)(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|)^t
\Bigg|\\
& \ge 
C(H)^{t+1}\times 
\Bigg|
p(p\beta_{1,1} + (1-p)\beta_{1,2})^t + 
(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})^t
\Bigg|.
\end{split}
\end{equation}
Now, there could be two reasons for why this inequality occurs:
\begin{enumerate}
    \item \emph{In-bracket cancellation:} For some large $K$ to be chosen later,
    \begin{equation}
    \label{eq:inbracketcancelation}
        \begin{split}
            & p\Bigg(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|\Bigg)^t \ge K^t \times
            p\Bigg|p\beta_{1,1} + (1-p)\beta_{1,2}\Bigg|^t \\
            & \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \text{or}\\
            & (1-p)\Bigg(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|\Bigg)^t \ge K^t \times
            (1-p)\Bigg|p\beta_{1,2} + (1-p)\beta_{2,2}\Bigg|^t
        \end{split}
    \end{equation}
    $.
    $
    \item \emph{Out-of-bracket cancellation:} For some very large $K,K_1$ to be chosen later,
    \begin{equation}
    \label{eq:outofbracketcancelation}
        \begin{split}
            & p\Bigg(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|\Bigg)^t \le K^t\times
            p\Bigg|p\beta_{1,1} + (1-p)\beta_{1,2}\Bigg|^t \\
            & \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \text{and}\\
            & (1-p)\Bigg(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|\Bigg)^t \le K^t\times 
            (1-p)\Bigg|p\beta_{1,2} + (1-p)\beta_{2,2}\Bigg|^t,\\
            & \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \text{but}\\
            & 
            K_1^t\times\Bigg|p\Bigg(p\beta_{1,1} + (1-p)\beta_{1,2}\Bigg)^t + 
            (1-p)\Bigg(p\beta_{1,2} + (1-p)\beta_{2,2}\Bigg)^t\Bigg|
            \\
            & \quad\quad\quad\quad\quad\le 
            p\Bigg|p\beta_{1,1} + (1-p)\beta_{1,2}\Bigg|^t + 
            (1-p)\Bigg|p\beta_{1,2} + (1-p)\beta_{2,2}\Bigg|^t
        \end{split}
    \end{equation}
    
\end{enumerate}
We analyse those two cases separately. In both cases, we use the cancellation conditions to give relationships between the parameters $p,\beta_{1,1}, \beta_{1,2}, \beta_{2,2}.$ We exploit these relationships to argue what the dominant community label assignments are to the expression $\ESW_{\SBM(p,1-p, \beta)}(H).$ We finish by comparing those dominant terms to the signed expectations of stars and 4-cycles. To do so, we need a very careful analysis based on the community assignments and presence of leaves in $H.$

\subsection{Preliminaries}
\begin{claim} $\ESW_{\SBM(p,1-p, \beta)}(\Star_t) = p[p\beta_{1,1} + (1-p)\beta_{1,2}]^t + 
(1-p)[p\beta_{1,2} + (1-p)\beta_{2,2}]^t.$    
\end{claim}
\begin{proof} Follows immediately by conditioning on the central vertex of the star.
\end{proof}

\begin{claim} $\ESW_{\SBM(p,1-p, \beta)}(C_4) =\Theta(\max(p^4\beta_{1,1}^4, p^2\beta_{1,2}^4, \beta_{2,2}^4)).$
\end{claim}
\begin{proof}
Explicitly, 
\begin{align*}
& \ESW_{\SBM(p,1-p, \beta)}(C_4) = 
p^4\beta_{1,1}^4 + 
4p^3(1-p)\beta_{1,1}^2\beta_{1,2}^2 + 
4p^2(1-p)^2 \beta_{1,1}\beta_{1,2}^2\beta_{2,2}\\
& + 
2p^2(1-p)^2 \beta_{1,2}^4 + 
4p(1-p)^3 \beta_{1,2}^2\beta_{2,2}^2 + 
(1-p)^4\beta_{2,2}^4.
\end{align*}
Observe that $|4p^2(1-p)^2 \beta_{1,1}\beta_{1,2}^2\beta_{2,2}|\le 
2p^3(1-p)\beta_{1,1}^2\beta_{1,2}^2 +
2p(1-p)^3\beta_{1,2}^2\beta_{2,2}^2
$ by AM-GM. Hence the above expression is between 
$p^4\beta_{1,1}^4 + 
2p^3(1-p)\beta_{1,1}^2\beta_{1,2}^2 +  
2p^2(1-p)^2 \beta_{1,2}^4 + 
2p(1-p)^3 \beta_{1,2}^2\beta_{2,2}^2 + 
(1-p)^4\beta_{2,2}^4$ and 
$p^4\beta_{1,1}^4 + 
6p^3(1-p)\beta_{1,1}^2\beta_{1,2}^2 +  
2p^2(1-p)^2 \beta_{1,2}^4 + 
6p(1-p)^3 \beta_{1,2}^2\beta_{2,2}^2 + 
(1-p)^4\beta_{2,2}^4.$ Similarly, 
observe that $0\le 2p^3(1-p)\beta_{1,1}^2\beta_{1,2}^2\le p^4\beta_{1,1}^4 + p^2(1-p)^2\beta_{1,2}^2.$ Using also that $1- p \in [1/2, 1)$ gives the desired conclusion.
\end{proof}

Now, observe that for any connected $H,$
\begin{align}
\label{eq:explicitH2SBM}
\ESW_{\SBM(p,1-p,\beta)}(H) = 
\sum_{K\subseteq V(H)}
p^{|K|}(1-p)^{|V(H)| - |K|}
\beta_{1,1}^{E(K,K)}
\beta_{1,2}^{E(K,V(H)\backslash K)}
\beta_{2,2}^{E(V(H)\backslash K, V(H)\backslash K)}.
\end{align}
\begin{claim}[Comparison with a non-negative model]
For any connected $H,$
$$
|\ESW_{\SBM(p,1-p,\beta)}(H)|\le |\ESW_{\SBM(p,1-p,|\beta|)}(H)|\le \max_{1\le t\le |V(H)|-1}
|\ESW_{\SBM(p,1-p,|\beta|)}(\Star_{t})|^{1/(t+1)}.
$$
\end{claim}
\begin{proof}
    By \cref{eq:explicitH2SBM}, 
    \begin{align*}
        & |\ESW_{\SBM(p,1-p,\beta)}(H)| \\
        & \le \Big|\sum_{K\subseteq V(H)}
p^{|K|}(1-p)^{|V(H)| - |K|}
\beta_{1,1}^{E(K,K)}
\beta_{1,2}^{E(K,V(H)\backslash K)}
\beta_{2,2}^{E(V(H)\backslash K), V(H)\backslash K)}\Big| \\
& \le \sum_{K\subseteq V(H)}
p^{|K|}(1-p)^{|V(H)| - |K|}
|\beta_{1,1}|^{E(K,K)}
|\beta_{1,2}|^{E(K,V(H)\backslash K)}
|\beta_{2,2}|^{E(V(H)\backslash K, V(H)\backslash K)]} \\
& = |\ESW_{\SBM(p,1-p,|\beta|)}(H)|.
    \end{align*}
This completes the first inequality. The second one follows immediately from \cref{sec:nonnegative}.
\end{proof}

Hence, if $H$ violates \cref{thm:2sbmtheorem}, it must be the case that 
\begin{equation}
\label{eq:starfailurecondition}
\begin{split}
&\Bigg|
p(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|)^t + 
(1-p)(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|)^t
\Bigg|\\
& \ge 
C(H)^{t+1}\times 
\Bigg|
p(p\beta_{1,1} + (1-p)\beta_{1,2})^t + 
(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})^t
\Bigg|.
\end{split}
\end{equation}

Now on, we assume that \cref{eq:starfailurecondition} holds. Then, one of the two conditions \cref{eq:inbracketcancelation} and \cref{eq:outofbracketcancelation} must hold. In particular, $|V(H)|\ge 3$ as the only connected graph on 2 vertices is $\Star_1.$

\subsection{The Case of In-Bracket Cancellation}
\label{sec:inbracketcancelation}
Suppose that \cref{eq:inbracketcancelation} holds. 

\begin{claim} If \cref{eq:starfailurecondition} and 
\cref{eq:inbracketcancelation} both hold,  $|\beta_{1,2}|\le C p|\beta_{1,1}|$  for some constant $C$ depending only on $K.$
\end{claim}
\begin{proof} 
There are two cases based on which of the inequalities in \cref{eq:inbracketcancelation} is satisfied. 

\medskip 

\textbf{Case 1)} First, suppose that $p(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|)^t\ge K^{t}\times \Big|
p(p\beta_{1,1} + (1-p)\beta_{1,2})^t\Big|.$ Then, 
$$
(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|)\ge K
\Big|
p\beta_{1,1} + (1-p)\beta_{1,2}\Big|\ge 
K\Big|
p|\beta_{1,1}| - (1-p)|\beta_{1,2}|
\Big|.
$$ 
A trivial calculation shows that $(1-p)|\beta_{1,2}|\in (1\pm \frac{2}{K-1})p|\beta_{1,1}|$ which is enough. 

\medskip

\textbf{Case 2)} Now, consider the other case. That is, 
$$
(1-p)(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|)^t\ge  K^t 
\Big|(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})^t
\Big|.
$$
Then, 
$p|\beta_{1,2}| + (1-p)|\beta_{2,2}|\ge K \Big|(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})^t
\Big|\ge K\Big|
p|\beta_{1,2}| - (1-p)|\beta_{2,2}|
\Big|.$ Again, $p|\beta_{1,2}|\in (1 \pm \frac{2}{K-1})(1- p)|\beta_{2,2}|.$  Hence, $(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|)\le 3p|\beta_{1,2}|,$ so 
$$
\Big|(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2}
\Big|\le \frac{1}{K}(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|)\le \frac{3}{K}p|\beta_{1,2}|
$$


Now, there are two cases. Either $|p\beta_{1,1} + (1- p)\beta_{1,2}|\le  \frac{1}{\sqrt{K}}(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|),$ which immediately implies  $(1-p)|\beta_{1,2}|\in (1\pm \frac{2}{\sqrt{K}-1})p|\beta_{1,1}|$ as in \textbf{Case 1)}. Or, 
\begin{align*}
&|p\beta_{1,1} + (1- p)\beta_{1,2}|>  \frac{1}{\sqrt{K}}(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|)\ge\frac{1}{\sqrt{K}}(1- p)|\beta_{1,2}|\ge \frac{1}{2\sqrt{K}}|\beta_{1,2}|\\
% & \ge \frac{\sqrt{K}}{3(1-p)}\frac{3}{K}p|\beta_{1,2}|\ge \frac{\sqrt{K}}{3}
% \Big|(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2}
% \Big|.
\end{align*}
This, however, means that 
\begin{align*}
    & \Bigg|
    p(p\beta_{1,1} + (1-p)\beta_{1,2})^t + 
(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})^t
    \Bigg|\\
    & \ge
    \Bigg|
    p(p\beta_{1,1} + (1-p)\beta_{1,2})^t\Bigg| - \Bigg| 
(1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})^t
    \Bigg|\\
    & \ge p \times \Big(\frac{1}{2\sqrt{K}}|\beta_{1,2}|\Big)^t - 
    (1- p)\Big(\frac{3}{K}p|\beta_{1,2}|\Big)^t\\
    & \ge \frac{p(1-p)^t|\beta_{1,2}|^t}{K^t}\ge 
    \frac{p|\beta_{1,2}|^t}{(2K)^t}
\end{align*}
for all $K\ge 128.$ Consider \cref{eq:starfailurecondition} (say $C(H) = (4K)^2$). Then, as $(p|\beta_{1,2}| + (1-p)|\beta_{2,2}|)\le 3p|\beta_{1,2}|,$ it must be the case that
\begin{align*}
    p(p|\beta_{1,1}| + (1-p)|\beta_{1,2}|)^t + (1-p)(3p|\beta_{1,2}|)^t\ge 
    (4K^2)^{t+1}
    \frac{p|\beta_{1,2}|^t}{(2K)^t}.
\end{align*}
For large enough $K\ge 128,$ this immediately implies that
$$
p|\beta_{1,1}| + (1-p)|\beta_{1,2}| \ge 
K\times |\beta_{1,2}|.
$$
Again, this implies $|\beta_{1,2}|\le Kp|\beta_{1,1}|.$ \end{proof}

It turns out that \cref{eq:inbracketcancelation} is enough to imply \cref{thm:2sbmtheorem}.

\begin{lemma}
\label{lem:whenbeta12issmall}
Suppose that $|\beta_{1,2}|\le C p|\beta_{1,1}|$  for some absolute constant $C.$ Then, 
for any connected graph $H,$ 
\begin{equation*}
    \begin{split}
        & |\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}\\
        & \le C(H)\times 
        \max \Big\{|\ESW_{\SBM(p,1-p, \beta)}(K)|^{1/|V(K)|}\; : \; K \text{ is a 4-cycle or a star with at most $V(H)$ vertices}\Big\}
        \end{split}
\end{equation*}
\end{lemma}
In the rest of the section, we prove \cref{lem:whenbeta12issmall}.
 We split the proof based on the weather $H$ is a tree or not. 

\subsubsection{Non-Tree Case}
Suppose that $H$ is connected and not a tree. Then, $H$ has at least $V(H)$ edges. Now, by \cref{eq:explicitH2SBM}, 
\begin{equation}
\label{eq:maximalbound}
    \begin{split}
        | \ESW_{\SBM(p,1-p, \beta)}(H)|\le 
        2^{|V(H)|}
        \max_{K\subseteq H}
        p^{|K|}
        |\beta_{1,1}|^{|E(K,K)|}
        |\beta_{1,2}|^{|E(K,V(H)\backslash K)|}
        |\beta_{2,2}|^{|E(V(H)\backslash K, V(H)\backslash K)|}
    \end{split}
\end{equation}
Now on, we will focus on a specific choice of $K.$ Suppose that $K$ is such that $H|_{K}$ has $a$ connected components and $|K| = t.$ Hence, $|E(K,K)|\ge a + t.$ Let $H|_{V(H)\backslash K}$ have $b$ connected components and $b+s$ vertices. Hence, 
$|E(H\backslash K, H\backslash K)|\ge s.$ Finally, observe that $|E(K,H\backslash K)|\ge a+b-1$ since $H$ is connected. There is at least one more edge besides that $a+b+t+s-1$ identified so far. Suppose that it is of teh type $|\beta_{i,j}|.$ Altogether,
\begin{equation*}
    \begin{split}
        & p^{|K|}
        |\beta_{1,1}|^{|E(K,K)|}
        |\beta_{1,2}|^{|E(K,H\backslash K)|}
        |\beta_{2,2}|^{|E(H\backslash K, H\backslash K)|}\\ 
        & \le p^{a+t}\times |\beta_{1,1}|^t\times |\beta_{1,2}|^{a+b-1}\times 
        |\beta_{2,2}|^s\times |\beta_{i,j}|\\
        & \le p^{a+ t + a + b - 1} \times |\beta_{1,1}|^{a + b + t -1}\times |\beta_{2,2}|^s \times |\beta_{i,j}|
    \end{split}
\end{equation*}
If $(i,j)\in \{(1,1), (1,2)\},$ then $a\ge 1$ (as label 1 exists) and $|\beta_{i,j}| = O(|\beta_{1,1}|).$ Thus, the above is expression is bounded by 
\begin{align*}
&p^{a + b + t } \times |\beta_{1,1}|^{a + b + t}\times |\beta_{2,2}|^s\\
&\le (p|\beta_{1,1}|)^{a + b + t}\times |\beta_{2,2}|^s\\
& \le |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{a+ b + t}{4}}\times 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{s}{4}}\\
&= |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)|}{4}},
\end{align*} which completes the proof.

If $(i,j) = (2,2),$ the above expression is bounded by 
$$
p^{t + a + b - 1} \times |\beta_{1,1}|^{a + b + t -1}\times |\beta_{2,2}|^{s + 1}
$$
and we argue similarly.

\subsubsection{The tree case}
Now, suppose that $H$ is a tree. Hence, it has two leaves $\ell_1,\ell_2.$ Now, we bound $|\ESW_{\SBM(p,1-p,\beta)}(H)|$ by conditioning on all the labels besides those of the two leaves. Namely, 
\begin{equation}
\label{eq:boundwiyhoutleavesinnerbrackets}
    \begin{split}
        &\Big| \ESW_{\SBM(p,1-p, \beta)}(H)\Big|\\
        &=  
        \sum_{K\subseteq V(H)\backslash\{\ell_1, \ell_2\}}
        p^{|K|}        
        \beta_{1,1}^{|E(K,K)|}
        \beta_{1,2}^{|E(K,H\backslash K)|}
        \beta_{2,2}^{|E(H\backslash K, H\backslash K)|}\\
        & \quad\quad\quad\quad\quad\quad\times (p\beta_{1,1} + (1-p)\beta_{2,2})^{P_1(K)}
        (p\beta_{1,2} + (1-p)\beta_{2,2})^{P_2(K)},
    \end{split}
\end{equation}
where $P_1(K)$ is the number of parents of $\ell_1, \ell_2$ with label $1$ according to $K$ and $P_2(K)$ with label 2 (in case of a common parent, we count it twice). Note that $P_1(K) + P_2(K) = 2.$ By AM-GM,
\begin{align*}
&|(p\beta_{1,1} + (1-p)\beta_{2,2})^{P_1(K)}
        (p\beta_{1,2} + (1-p)\beta_{2,2})^{P_2(K)}|\\
&\le 
p^{-\indicator[a\ge 1]}\Bigg(
(p\beta_{1,1} + (1-p)\beta_{2,2})^2 + 
(p\beta_{1,2} + (1-p)\beta_{2,2})^2\Bigg) \le 
p^{-\indicator[a\ge 1]}\ESW_{\SBM(p,1-p,\beta)}(\Star_2).
\end{align*}
The $\indicator[a\ge 1]$ factor comes from the fact that if $a = 0,$ then $P_1(K) = 0.$   
Combining with \cref{eq:boundwiyhoutleavesinnerbrackets},
\begin{equation}
\begin{split}
    &\Big| \ESW_{\SBM(p,1-p, \beta)}(H)\Big|\le\\
    &2^{|V(H)|-2}\max_{K\subseteq V(H)\backslash\{\ell_1, \ell_2\}}
        p^{|K|}        
        |\beta_{1,1}|^{|E(K,K)|}
        |\beta_{1,2}|^{|E(K,H\backslash K)|}
        |\beta_{2,2}|^{|E(H\backslash K, H\backslash K)|}\\
        & \quad\quad\quad\quad\quad\quad\quad\times p^{-\indicator[a\ge 1]}|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|
\end{split}
\end{equation}
Again, we denote by $a$ the connected components of $K,$ by $a + t$ its vertices, by $b$ the connected components of $V(H)\backslash K$ and by $b + t$ the number of vertices. We obtain the bound:
\begin{align}
& p^{a + t}
|\beta_{1,1}|^t 
|\beta_{1,2}|^{a + b - 1}
|\beta_{2,2}|^s
p^{-\indicator[a\ge 1]}|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\\
& \le 
p^{a + t -1 + a + b - \indicator[a\ge 1]}
|\beta_{1,1}|^{a+ b + t -1}
|\beta_{2,2}|^s
|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|.
\end{align}
Using that $a-\indicator[a\ge 1]\ge 0,$ we bound
\begin{align}
&(p|\beta_{1,1}|)^{a+ b + t -1}
   |\beta_{2,2}|^s
|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\\
& \le 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{a +b + t -1}{4}}
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{s}{4}
|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\\
& = 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{|V(H)| - 3}{4}
|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\\
& = 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{|V(H)| }{4}\times 
\Bigg(\frac{|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|}{|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{3}{4}}\Bigg).
\end{align}
Hence, 
\begin{align}
\label{eq:cycleand2starinnercancelation}
   |\ESW_{\SBM(p,1-p,\beta)}(H)|^{1/|V(H)|}\lesssim
   |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}\times 
   \Bigg(\frac{|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|}{|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{3}{4}}\Bigg)^{1/|V(H)|}.
\end{align}
If $ \Bigg(\frac{|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|}{|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{3}{4}}\Bigg)\le 1,$ the LHS of \cref{eq:cycleand2starinnercancelation} is bounded by $|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}.$ If 
$ \Bigg(\frac{|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|}{|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^\frac{3}{4}}\Bigg)\ge 1,$ the LHS of \cref{eq:cycleand2starinnercancelation} is decreasing in $|V(H)|$ and is hence minimized for $|V(H)| = 3.$ In this case, the resulting bound is 
$|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|^{1/3}.$
\subsection{The Case of Out-of-Bracket Cancellation}
\label{sec:outofbracketcancelation}
Now, suppose that \cref{eq:starfailurecondition} holds in the case of \cref{eq:outofbracketcancelation}. Additionally, we assume that $|\beta_{1,2}|\ge Cp|\beta_{1,1}|$ as we otherwise can invoke \cref{lem:whenbeta12issmall}. In particular, 
$p|\beta_{1,1}| + (1-p)|\beta_{1,2}| \le (C+1)|\beta_{1,2}|).$ By \cref{eq:outofbracketcancelation}
\begin{align}
\label{eq:boundonpbeta11plusbeta22}
\frac{1}{C_1}|\beta_{1,2}|\le |p\beta_{1,1} + (1-p)\beta_{1,2}|\le C_1|\beta_{1,2}|\text{ for some absolute constant }C_1.\end{align}

Note that \cref{eq:outofbracketcancelation} immediately implies that $p\Bigg(p\beta_{1,1} + (1-p)\beta_{1,2}\Bigg)^t, 
            (1-p)\Bigg(p\beta_{1,2} + (1-p)\beta_{2,2}\Bigg)^t$ have different signs. In particular, $t$ is odd.
            
Next, we will show that unless $p\ge |\beta_{1,2}|,$ $\Star_{t+1}$ dominates $H.$

\begin{lemma}
\label{lem:whenbeta12gep}
Suppose that \cref{eq:starfailurecondition} holds and $p \le K |\beta_{1,2}|.$ Then, 
$$
|\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}\le 
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{t+1})|^{1/(t+2)},
$$    
\end{lemma}
\begin{proof}
    For brevity, denote $\mu = p\beta_{1,1} + (1-p)\beta_{1,2},\lambda = 
p\beta_{1,2} + (1-p)\beta_{2,2}.$ We know that $K|\mu|\ge p|\beta_{1,1}| + (1-p)|\beta_{1,2}| $ and 
$K|\lambda|\ge p|\beta_{1,2}| + (1-p)|\beta_{2,2}|$ under \cref{eq:outofbracketcancelation}. However, 
$K_1^t\times |p\mu^t + (1-p)\lambda^t|\le \Big(p|\mu|^t + (1-p)|\lambda|^t\Big).$ In particular, this means
$K_1^t\times \Big|p|\mu|^t - (1-p)|\lambda|^t\Big|\le  \Big(p|\mu|^t + (1-p)|\lambda|^t\Big),$ so 
$p|\mu|^t\in (1\pm 1/2)(1-p)|\lambda|^t$ for large enough $K_1.$  By \cref{eq:boundonpbeta11plusbeta22}, also 
$|\mu|\ge \frac{1}{C_1}|\beta_{1,2}|\ge \frac{p}{KC_1}.$

Now, since $t+1$ is even and $\mu \ge \frac{p}{KC_1},$ $(p\mu^{t+1})^{1/(t+2)}\ge (p|\mu|^t)^{1/(t+1)}(KC_1)^{-\frac{1}{(t+1)(t+2)}}.$ Altogether, 
\begin{equation*}
    \begin{split}
        & |\ESW_{\SBM(p,1-p, \beta)}(\Star_{t+1})|^{1/(t+2)}\\
        & = |p\mu^{t+1} + (1-p)\lambda^{t+1}|^{1/(t+2)}
         \ge |p\mu^{t+1}|^{1/(t+2)}
        \ge (KC_1)^{-\frac{1}{(t+1)(t+2)}} |p\mu^t|^{1/(t+1)}\\
        & \ge (KC_1)^{-\frac{1}{(t+1)(t+2)}}\Big(\frac{1}{3}\big( p|\mu|^t + (1-p)|\lambda|^t\big)\Big)^{1/(t+1)}\\
        & \ge \frac{1}{3^{1/(t+1)}(KC_1)^{\frac{1}{(t+1)(t+2)}}}
        |\ESW_{\SBM(p,1-p, |\beta|)}(\Star_{t})|^{1/(t+1)}\gtrsim 
        |\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}
    \end{split}
\end{equation*}
\end{proof}

Now on, we 
\begin{align}
\label{eq:beta12issmall}
\text{ Assume that }|\beta_{1,2}|\le p.
\end{align}
\subsubsection{The case of $t>1$}
When $|\beta_{1,2}|<p,$ we can run the same argument showing that 
$$
|\ESW_{\SBM(p,1-p, \beta)}(\Star_{t-1})|^{1/t}\gtrsim 
|\ESW_{\SBM(p,1-p, |\beta|)}(\Star_{t})|^{1/(t+1)}
\gtrsim
        |\ESW_{\SBM(p,1-p, \beta)}(H)|^{1/|V(H)|}.$$
Of course, this works as long as $t>2.$ Hence, now on, we assume that $t = 1.$
\subsubsection{Characterizing the SBM when $t = 1$}
All that is left is the case $t = 1.$ For convenience, we restate and recall what we know.
\begin{enumerate}
    \item $p|\beta_{1,1}| + (1-p)|\beta_{1,2}|\le K \times|p\beta_{1,1} + (1-p)\beta_{1,2}|$ and 
    $p|\beta_{1,2}| + (1-p)|\beta_{2,2}|\le K \times|p\beta_{1,2} + (1-p)\beta_{2,2}|,$ but 
    \begin{align*}
    & K_1\times |p(p\beta_{1,1} + (1-p)\beta_{1,2}) + (1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})|\\
    & \le
    p|p\beta_{1,1} + (1-p)\beta_{1,2}| + (1-p)|p\beta_{1,2} + (1-p)\beta_{2,2}|
    \end{align*}
    by \cref{eq:outofbracketcancelation}.
    \item $|\beta_{1,2}|\ge Cp|\beta_{1,1}|$ as otherwise \cref{lem:whenbeta12issmall} gives \cref{thm:2sbmtheorem}.
    \item $|\beta_{1,2}|\le p$ as otherwise \cref{lem:whenbeta12gep} implies the result.
\end{enumerate}
Observe that under the above assumptions, $|p(p\beta_{1,1} + (1-p)\beta_{1,2})|\le C'p|\beta_{1,2}|$ for some $C'.$ Furthermore,
\begin{align*}
    & 
    p|p\beta_{1,1} + (1-p)\beta_{1,2}| + (1-p)|p\beta_{1,2} + (1-p)\beta_{2,2}|\\
    & \ge K_1\times|p(p\beta_{1,1} + (1-p)\beta_{1,2}) + (1-p)(p\beta_{1,2} + (1-p)\beta_{2,2})|\\
    & \ge K_1\times\Big|
    p|p\beta_{1,1} + (1-p)\beta_{1,2}| - 
    (1-p)|p\beta_{1,2} + (1-p)\beta_{2,2}|
    \Big|.
\end{align*}
Immediately, for $K_1\ge 3,$ we obtain 
$$(1-p)|p\beta_{1,2} + (1-p)\beta_{2,2}|\le p|p\beta_{1,1} + (1-p)\beta_{1,2}| \le 2C'p|\beta_{1,2}|.$$
As $(1-p)|p\beta_{1,2} + (1-p)\beta_{2,2}|\ge Kp|\beta_{1,2}| + K(1-p)|\beta_{2,2}|,$ this implies that
\begin{enumerate}
    \item [4.] $|\beta_{2,2}|\le K'p|\beta_{1,2}|$ for some absolute constant $K'.$ 
\end{enumerate}
Finally, this immediately implies that $|p\beta_{1,2} + (1-p)\beta_{2,2}| = \Theta(p|\beta-{1,2}|).$ In turn,
    \begin{align}
    \label{eq:starexpectationsint1outbrackets}
        \text{5.} \quad\quad\ESW_{\SBM(p,1-p,\beta)}(\Star_t) = \Theta(p|\beta_{1,2}|^t) = 
        \Theta(p((1-p)\beta_{1,1} + p\beta_{1,2})^t)
        \text{ for any even }t\ge 2.
    \end{align}

Now, we will carry out a similar analysis as in \cref{sec:inbracketcancelation}, but we will need a more careful analysis of the leaves. Namely, Suppose that $L\subseteq V(H)$ is the set of leaves and for $K\subseteq V(H)\backslash L,$ the number of leaves with parents of label $1$ is $L_1(K)$ and with parents of label $2$ is $L_2(K).$ Hence, 
\begin{equation}
\begin{split}
    &|\ESW_{\SBM(p,1-p,\beta)}(H)|\\
    & = \Bigg|\sum_{K\subseteq V(H)\backslash L}
    p^{|K|}(1- p)^{|V(H)| - |L| - |K|}\times\\
    &\quad\quad\quad\quad\quad
    \beta_{1,1}^{|E(K,K)|}
    \beta_{1,2}^{|E(K,V(H)\backslash (K\cup L))|}
    \beta_{2,2}^{|E(V(H)\backslash (K\cup L),  V(H)\backslash (K\cup L))|}
    (p\beta_{1,1} + \beta_{1,2})^{L_1(K)}
    (p\beta_{1,2} + (1-p)\beta_{2,2})^{L_2(K)}
    \Bigg|\\
    & \le 2^{|V(H)|}\max_Kp^{|K|}
    |\beta_{1,1}|^{|E(K,K)|}
    |\beta_{1,2}|^{|E(K,V(H)\backslash (K\cup L))|}\\
    & \quad\quad\quad\quad\quad \times
    |\beta_{2,2}|^{|E(V(H)\backslash (K\cup L), V(H)\backslash (K\cup L))|}
    |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}
    \end{split}
\end{equation}
Again, let $K$ have $a$ connected components and $a+t$ vertices and $H|_{V(H)\backslash (K\cup L)}$ have $b$ connected components and $b+s$ vertices. In particular, 
$$
|V(H)| = a + b + t + s + L_1(K) + L_2(K).
$$
For a fixed $K,$ the above expression is at most 
$$
p^{a+t}|\beta_{1,1}|^t |\beta_{1,2}|^{a + b - 1}
|\beta_{2,2}|^s 
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}.
$$
Using that $|\beta_{2,2}|\le K'p|\beta_{1,2}|,$ the above expression is, up to absolute constants, bounded by 
\begin{align}
\label{eq:comparisoninoutofbracketscase}
    p^{a+t +s + L_2(K)}|\beta_{1,1}|^t |\beta_{1,2}|^{a + b - 1 + s + L_2(K)}
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
\end{align}
We now analyze two cases based on which of the two quantities $|\beta_{1,1}|\sqrt{p}, |\beta_{1,2}|$ is larger. 
\subsubsection{The case $|\beta_{1,1}|\sqrt{p}\le |\beta_{1,2}|$}
\label{sec:squarerootcomparison }
Using $|\beta_{1,1}|\sqrt{p}\le |\beta_{1,2}|$, we bound \cref{eq:comparisoninoutofbracketscase}
by
$$
p^{a+t/2 +s + L_2(K)} |\beta_{1,2}|^{a + b - 1 + s + L_2(K) + t}
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
$$
\paragraph{Case 1) $L_1(K)\le 2.$}
Using that $p|\beta_{1,1}| = O(|\beta_{1,2}|),$ the above expression is, up to constant factors, bounded by 
\begin{align*}
 & p^{a+t/2 +s + L_2(K)}|\times  |\beta_{1,2}|^{a + b - 1 + s + L_2(K) +t + L_1(K)}\\
 & \lesssim 
  p^{a+t/2 +s + L_2(K)-1}|\times  |\beta_{1,2}|^{a + b - 3 + s + L_2(K) +t+ L_1(K)}\times 
  \ESW_{\SBM(p,1-p,\beta)}(\Star_2)
\end{align*}
where we used \cref{eq:starexpectationsint1outbrackets}.
 Now, suppose that 
 $$
 a+t/2 +s + L_2(K)-1\ge \frac{1}{2}(a + b - 3 + s +t+ L_2(K) + L_1(K)).
 $$
 Then, the above expression is bounded by 
\begin{align*}
 & (\sqrt{p}|\beta_{1,2}|)^{a + b - 3 + s + L_2(K) +t+ L_1(K)}\times 
  \ESW_{\SBM(p,1-p,\beta)}(\Star_2)\\
  & \lesssim 
  |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)|-3}{4}}\times 
  |\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|.
\end{align*}
Again, this expression is smaller than $\max(|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}, 
  |\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|^{1/3})^{|V(H)|}.$

Hence, the interesting case is 
\begin{align*}
&a+t/2 +s + L_2(K)-1< \frac{1}{2}(a + b - 3 + s + L_2(K) + t+L_1(K))\quad\quad\quad\Longleftrightarrow\\
&
a + s + L_2(K) + 1< b + L_1(K)\quad\quad\quad\Longleftrightarrow\\
& a + s + L_2(K) + 2\le b + L_1(K).
\end{align*}
Since $L_1(K)\le 2,$ it follows that $b = a + s + L_2(K) + r$ for some $r\ge 0.$  In particular, this means that $H|_{V(H)\backslash (K\cup L_1(K))}$ has at least $R \ge b - s-L_2(K) = a +r$ singletons. Indeed, note that $H|_{V(H)\backslash (K\cup L)}$ has $b$ connected components and $b+ s$ vertices. Hence, at least $b-s$ of the vertices in $H|_{V(H)\backslash (K\cup L)}$ are isolated. These same vertices are not isolated in $H|_{V(H)\backslash (K\cup L_1(K))}$ if and only if they have a neighbour in $L_2(K).$ As each vertex in $L_2(K)$ is a leaf, there are at most $L_2(K)$ such of them. Hence, at least $b - s - L_2(K) = a  + r$ of the vertices in $V(H)\backslash (K\cup L)$
are isolated in 
$H|_{V(H)\backslash (K\cup L_1(K))}.$ Denote these vertices by $\mathcal{S},$ so $|\mathcal{S}|\ge a ++ r.$

Now consider 
$
H|_{V(H)\backslash L}.
$ This is a connected graph since $H$ is connected and $L$ is the set of leaves. Hence, each connected components in $H|_{V(H)\backslash (L\cup K)}$ has at least one edge to a vertex in $K.$ If, furthermore, this connected component is one of the vertices in $\mathcal{S},$ it must have at least $2$ edges to $K.$ At least one edge due to connectivity and at least one more as the vertices of $\mathcal{S}$ are not leaves ($\mathcal{S}\subseteq V(H)\backslash (K\cup L_1(K)$) and they don't have any edges to other vertices in $V(H)\backslash (K\cup L_1(K))$ due to being isolated, and in $L_1(K)$ due to the fact that the parents of leaves in $L_1(K)$ are all in $K.$ Altogether, this means that the number of edges between $K$ and $V(H)\backslash (L\cup K)$ is at least 
$$
2|\mathcal{S}| + (b - |\mathcal{S}|)\ge 
b + |\mathcal{S}|\ge 
b + a + r .
$$ Note that all of these edges are of type $(1,2).$
Thus, we can bound
\begin{equation*}
\begin{split}
    &|\ESW_{\SBM(p,1-p,\beta)}(H)|\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t\times |\beta_{1,2}|^{b + a + r }\times 
    |\beta_{2,2}|^{s}\times 
    |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}\\
    & \lesssim 
    p^{a + t}|\beta_{1,2}|^tp^{-t/2}
    |\beta_{1,2}|^{b + a + r }\times 
    |\beta_{1,2}|^{s}p^s
    |\beta_{1,2}|^{L_1(K)}
    |\beta_{1,2}|^{L_2(K)}
    p^{L_2(K)}\\
    & \lesssim 
    p^{a + t/2 + s + L_2(K)}
    |\beta_{1,2}|^{t + b + a + r +s+L_1(K) + L_2(K)}\\
    & \lesssim 
    p^{a + t/2 + s + L_2(K) -1}\times 
    |\beta_{1,2}|^{t + b + a + s+L_1(K) + L_2(K) - 3}\times p|\beta_{1,2}|^{2}\times 
    |\beta_{1,2}|^{1 + r}\\
    & \lesssim 
    p^{a + t/2 + s + L_2(K) + r}
    \times 
    |\beta_{1,2}|^{t + b + a + s+L_1(K) + L_2(K) - 3}\times p|\beta_{1,2}|^{2},
\end{split}
\end{equation*}
where in the last line we used that $|\beta_{1,2}|\le p.$ Now, observe that 
$$
a + t/2 + s + L_2(K) + r\ge \frac{1}{2}(t + b + a + s+L_1(K) + L_2(K) - 3)
$$
since this is equivalent to 
$$
a + s + L_2(K) + 2r + 3\ge b + L_1(K),
$$
but $a + s + L_2(K) + r = b,r + 3\ge 3>L_1(K).$ Altogether, the above expression is bounded by 
$$
(\sqrt{p}|\beta_{1,2}|)^{t + b + a + s+L_1(K) + L_2(K) - 3}\times p|\beta_{1,2}|^{2}\lesssim 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)|-3}{4}}
\times 
|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|.
$$

\paragraph{Case 2) $L_1(K)\ge 3.$} Let $\xi\in \{0,1\}$ be such that $L_1(K) -\xi$ is even. We bound
\cref{eq:comparisoninoutofbracketscase} bu 
\begin{align*}
& p^{a+t +s + L_2(K)}|\beta_{1,1}|^t |\beta_{1,2}|^{a + b - 1 + s + L_2(K)}
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}\\
& \lesssim 
p^{a+t +s + L_2(K)}|\beta_{1,2}|^tp^{-t/2} |\beta_{1,2}|^{a + b - 1 + s + L_2(K)}
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)-\xi}|\beta_{1,2}|^\xi\\
& \lesssim 
p^{a+t/2 +s + L_2(K)}
|\beta_{1,2}|^{a + b - 1 + s + L_2(K) + t + \xi}
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|.
\end{align*}
Again, we consider two cases. 

\textbf{Case 2.1)}If 
\begin{align*}
& a+t/2 +s + L_2(K)\ge 
\frac{1}{2}(a + b - 1 + s + L_2(K) + t + \xi)\quad\quad\quad\Longleftrightarrow
& a + s + L_2\ge b + \xi - 1,
\end{align*}
the last expression is bounded by 
\begin{align*}
& |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)| - L_1(K) -1 + \xi}{4}}
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})| \\
& = 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)|}{4}}\times \Bigg(
\frac{\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})}{\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{L_1(K)-\xi + 1}{4}}}
\Bigg)\\
&\le  \max(|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}, 
  |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|^{1/(L_1(K)-\xi + 1)})^{|V(H)|}.
\end{align*}
The last equality follows from analysing $\frac{\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})}{\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{L_1(K)-\xi + 1}{4}}}.$ If this is less than 1, teh result is immediate. Else, 
$$
\Bigg(
\frac{\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})}{\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{L_1(K)-\xi + 1}{4}}}
\Bigg)^{1/|V(H)|}
$$
is decreasing in $|V(H)|,$ but $|V(H)|\ge L_1(K) + 1\ge L_1(K) + 1 - \xi. $


\textbf{Case 2.2) }Otherwise, 
\begin{align*}
& a+t/2 +s + L_2(K)< 
\frac{1}{2}(a + b - 1 + s + L_2(K) + t + \xi)\quad\quad\quad\Longleftrightarrow\\
& a + s + L_2(K)< b + \xi - 1,
\end{align*}
so $b + \xi \ge a + s + L_2 + 2.$ Since As in Case 1), we can set $b+ \xi = a  + s+ L_2(K) + r,$ where $r\ge 2.$ We use the same argument as in Case  1) to argue that there are at least 
$b + a + r - \xi$ edges between $K$ and $V(H)\backslash (K\cup L).$ We bound
\begin{equation*}
\begin{split}
    &|\ESW_{\SBM(p,1-p,\beta)}(H)|\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t\times |\beta_{1,2}|^{b + a + r - \xi }\times 
    |\beta_{2,2}|^{s}\times 
    |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}\\
    & \lesssim 
    p^{a + t}|\beta_{1,2}|^tp^{-t/2}
    |\beta_{1,2}|^{b + a + r -\xi}\times 
    |\beta_{1,2}|^{s}p^s
    p^{-1}|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\times |\beta_{1,2}|^\xi
    |\beta_{1,2}|^{L_2(K)}
    p^{L_2(K)}\\
    & \lesssim 
    p^{a + t/2 + s + L_2(K)-1}
    |\beta_{1,2}|^{t + b + a + r +s+L_2(K)}\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|
    \\
    & \lesssim 
    p^{a + t/2 + s + L_2(K) + r - \xi}
    |\beta_{1,2}|^{t + b + a  +s+L_2(K) + \xi - 1}\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|.
\end{split}
\end{equation*}
where we used $|\beta_{1,2}|\lesssim p.$ Now, observe that 
\begin{align*}
    & a + t/2 + s + L_2(K) + r - \xi\ge 
    \frac{1}{2}(t + b + a  +s+L_2(K) + \xi - 1)\quad\quad\quad\Longleftrightarrow\\
    & a + s + L_2(K) + 2r +1\ge b + 3\xi,
\end{align*}
but $b+ \xi = a + s + L_2(K) + r$ and $r + 1\ge 3\ge 2\xi.$ Altogether, this means that the above expression is at most 
$$
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)| - L_1(K) -1 + \xi}{4}}\times
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|
$$


\subsubsection{The case $|\beta_{1,1}|\sqrt{p}> |\beta_{1,2}|$}
We consider the same two cases based on $L_1(K).$

\paragraph{Case 1) $L_1(K)\le 2.$}
We bound the expression in  \cref{eq:comparisoninoutofbracketscase} by 
\begin{align*}
    & p^{a+t +s + L_2(K)}|\beta_{1,1}|^t |\beta_{1,2}|^{a + b - 1 + s + L_2(K)}
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}\\
& \lesssim p^{a+t +s + L_2(K)}|\beta_{1,1}|^t \times 
|\beta_{1,2}|^{a + b - 1 + s + L_2(K)}\times 
|\beta_{1,2}|^{L_1(K)}\\
& \lesssim 
p^{a+t +s + L_2(K) -1}\times 
|\beta_{1,1}|^t \times 
|\beta_{1,2}|^{a + b + s + L_2(K) + L_1(K) - 3}\times 
p|\beta_{1,2}|^2\\
& \lesssim
p^{a+t +s + L_2(K) -1}\times 
|\beta_{1,1}|^t \times 
|\beta_{1,1}|^{a + b + s + L_2(K)+ L_1(K) - 3}p^{(a + b + s + L_2(K) - 3)/2}\times 
p|\beta_{1,2}|^2\\
& \lesssim
p^{a+t +s + L_2(K) -1 + \frac{1}{2}(a + b + s + L_2(K)+ L_1(K) - 3)}|\beta_{1,1}|^{t + a + b + s + L_2(K)+ L_1(K) - 3}\times \ESW_{\SBM(p,1-p,\beta)}(\Star_{2})
\end{align*}
If 
\begin{align*}
    & a+t +s + L_2(K) -1 + \frac{1}{2}(a + b + s + L_2(K)+ L_1(K) - 3)\ge 
    t + a + b + s + L_2(K)+ L_1(K) - 3\Longleftrightarrow\\
    & a + s + L_2 + 1\ge b + L_1,
\end{align*}
then going back we have 
\begin{align*}
    & p^{a+t +s + L_2(K) -1 + \frac{1}{2}(a + b + s + L_2(K)+ L_1(K) - 3)}|\beta_{1,1}|^{t + a + b + s + L_2(K)+ L_1(K) - 3}\times \ESW_{\SBM(p,1-p,\beta)}(\Star_{2})\\
    & \le 
    (p|\beta_{1,1}|)^{|V(H)|-3}
    \ESW_{\SBM(p,1-p,\beta)}(\Star_{2})\\
    & \le 
    \ESW_{\SBM(p,1-p,\beta)}(C_4)^{\frac{|V(H)|-3}{4}}\times
    \ESW_{\SBM(p,1-p,\beta)}(\Star_{2})\\
    & \le 
    \max(|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}, 
  |\ESW_{\SBM(p,1-p,\beta)}(\Star_{2})|^{1/3})^{|V(H)|}.
\end{align*}
Otherwise, 
$a + s + L_2 + 1< b + L_1\le b + 2,$ so 
$b  = a + s + L_2 + r,$ where $r\ge 0.$ Again, using the argument of counting isolated vertices, we have 
\begin{equation*}
\begin{split}
    &|\ESW_{\SBM(p,1-p,\beta)}(H)|\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t\times |\beta_{1,2}|^{b + a + r}\times 
    |\beta_{2,2}|^{s}\times 
    |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t\times |\beta_{1,2}|^{b + a + r}\times 
    |\beta_{1,2}|^{s}p^s\times 
    |\beta_{1,2}|^{L_1(K)}
    |\beta_{1,2}|^{L_2(K)}p^{L_2(K)}\\
    & \lesssim 
    p^{a + t + s  + L_2(K)}\times |\beta_{1,1}|^t\times 
    |\beta_{1,2}|^{b +a + r + s + L_1(K) + L_2(K)}\\
    & \lesssim p^{a + t + s  + L_2(K) + r}
    |\beta_{1,1}|^t\times 
    |\beta_{1,2}|^{b +a + s + L_1(K) + L_2(K)}\\
    & \lesssim p^{a + t + s  + L_2(K) + r}
    |\beta_{1,1}|^t\times 
    |\beta_{1,2}|^{b +a + s + L_1(K) + L_2(K) - 3}p|\beta_{1,2}|^2\\
    & \lesssim p^{a + t + s  + L_2(K) + r + \frac{1}{2}(b +a + s + L_1(K) + L_2(K)-3)}
    |\beta_{1,1}|^{t + b +a + s + L_1(K) + L_2(K)-3}p|\beta_{1,2}|^2.\\
\end{split}
\end{equation*}
Now, observe that 
\begin{align*}
    & a + t + s  + L_2(K) + r + \frac{1}{2}(b +a + s + L_1(K) + L_2(K)-3)\ge t + b +a + s + L_1(K) + L_2(K)-3\quad\quad\quad\Longleftrightarrow\\
    & 3 + 2 r + a + s + L_2(K)\ge b + L_1.
\end{align*}
This is correct as $r + a + s + L_2(K)\ge b, 3 + r \ge 3\ge L_2(K).$ Hence, the above expression is bounded by 
$$
(p|\beta_{1,1}|)^{t + b +a + s + L_1(K) + L_2(K)-3}p|\beta_{1,2}|^2\lesssim 
|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)|-3}{4}}\times 
|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|.
$$

\paragraph{Case 2) $L_1(K)> 2.$}
Let $\xi \in \{0,1\}$ be such that $L_1(K)-\xi$ is even. Then, we bound the expression in  \cref{eq:comparisoninoutofbracketscase} by 
\begin{align*}
& p^{a+t +s + L_2(K)}|\beta_{1,1}|^t |\beta_{1,2}|^{a + b - 1 + s + L_2(K)}
|p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}\\
& \lesssim
p^{a+t +s + L_2(K)-1}|\beta_{1,1}|^t \times |\beta_{1,2}|^{a + b - 1 + s + L_2(K)}\times 
p |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)-\xi}|\times |\beta_{1,2}|^\xi\\
& \lesssim
p^{a+t +s + L_2(K)-1}|\beta_{1,1}|^t \times |\beta_{1,2}|^{a + b - 1 + s + L_2(K)+\xi}\times 
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K) - \xi})|\\
& \lesssim p^{a+t +s + L_2(K)-1}|\beta_{1,1}|^t \times |\beta_{1,1}|^{a + b - 1 + s + L_2(K)+\xi}p^{\frac{1}{2}(a + b - 1 + s + L_2(K)+\xi)}\times 
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K) - \xi})|\\
& \lesssim 
p^{a+t +s + L_2(K)-1 + \frac{1}{2}(a + b - 1 + s + L_2(K)+\xi)}|\beta_{1,1}|^{t +a + b - 1 + s + L_2(K)+\xi }\times 
|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K) - \xi})|.
\end{align*}
Again, note that if 
\begin{align*}
    & a+t +s + L_2(K)-1 + \frac{1}{2}(a + b - 1 + s + L_2(K)+\xi)\ge 
    t +a + b - 1 + s + L_2(K)+\xi \quad\quad\quad\Longleftrightarrow\\
    & a - 1 + s + L_2(K)\ge b + \xi, 
\end{align*}
the above expression is at most 
\begin{align*}
    & (p |\beta_{1,1}|)^{t +a + b - 1 + s + L_2(K)+\xi}\times |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K) - \xi})|\\
    & \lesssim 
    |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)| - L_1(K) - 1 + \xi}{4}}\times |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K) - \xi})|\le \\
    & \le \max(|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}, 
  |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|^{1/(L_1(K)-\xi + 1)})^{|V(H)|}.
\end{align*}

Otherwise, $a - 1 + s + L_2(K)< b + \xi,$ so $b + \xi = a + s + L_2(K) + r,$ where $r\ge 0.$ Using the isolated-vertices argument, 
\begin{equation*}
\begin{split}
    &|\ESW_{\SBM(p,1-p,\beta)}(H)|\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t\times |\beta_{1,2}|^{b + a + r - \xi }\times 
    |\beta_{2,2}|^{s}\times 
    |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t
    |\beta_{1,2}|^{b + a + r -\xi}\times 
    |\beta_{1,2}|^{s}p^s
    p^{-1}
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\times |\beta_{1,2}|^\xi
    |\beta_{1,2}|^{L_2(K)}
    p^{L_2(K)}\\
    & \lesssim 
    p^{a + t + s + L_2(K)-1}\times 
    |\beta_{1,1}|^{t}\times 
    |\beta_{1,2}|^{b + a + r+ s +L_2(K)}\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K)-1}\times 
    |\beta_{1,1}|^{t}\times 
    |\beta_{1,2}|^{b + a + s +L_2(K)+\xi - 1}p^{r + 1-\xi}\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K) + r-\xi}
     |\beta_{1,1}|^{t}\times 
    |\beta_{1,1}|^{b + a + s +L_2(K)+\xi - 1}
    p^{\frac{1}{2}(b + a + s +L_2(K)+\xi - 1)}
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K) + r-\xi + \frac{1}{2}(b + a + s +L_2(K)+\xi - 1)}
    |\beta_{1,1}|^{t + b + a + s +L_2(K)+\xi - 1}
    \times
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|
\end{split}
\end{equation*}
Now, 
\begin{align*}
    & a + t + s + L_2(K) + r-\xi + \frac{1}{2}(b + a + s +L_2(K)+\xi - 1)\ge 
    t + b + a + s +L_2(K)+\xi - 1 \quad\quad\quad\Longleftrightarrow\\
    & 
\end{align*}

\begin{equation*}
\begin{split}
    &|\ESW_{\SBM(p,1-p,\beta)}(H)|\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t\times |\beta_{1,2}|^{b + a + r - \xi }\times 
    |\beta_{2,2}|^{s}\times 
    |p\beta_{1,1} + \beta_{1,2}|^{L_1(K)}
    |p\beta_{1,2} + (1-p)\beta_{2,2}|^{L_2(K)}\\
    & \lesssim 
    p^{a + t}|\beta_{1,1}|^t
    |\beta_{1,2}|^{b + a + r -\xi}\times 
    |\beta_{1,2}|^{s}p^s
    p^{-1}
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\times |\beta_{1,2}|^\xi
    |\beta_{1,2}|^{L_2(K)}
    p^{L_2(K)}\\
    & \lesssim 
    p^{a + t + s + L_2(K)-1}\times 
    |\beta_{1,1}|^{t}\times 
    |\beta_{1,2}|^{b + a + r+ s +L_2(K)}\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K)-1}\times 
    |\beta_{1,1}|^{t}\times 
    |\beta_{1,2}|^{b + a + r+ s +L_2(K)-3}\times p\beta_{1,2}^2\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K)-1}\times 
    |\beta_{1,1}|^{t}\times 
    |\beta_{1,2}|^{b + a + r+ s +L_2(K)-3}\times |\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K)-1 + 1 + r-\xi}\times 
    |\beta_{1,1}|^{t}\times 
    |\beta_{1,2}|^{b + a + s +L_2(K)-4 + \xi}\times\\
    & \quad\quad\quad\quad\quad\quad\quad\quad|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K)+ r-\xi}\times 
    |\beta_{1,1}|^{t + b + a + s +L_2(K)-4 + \xi}\times 
    p^{\frac{1}{2}(b + a + s +L_2(K)-4 + \xi)}\times\\
    & \quad\quad\quad\quad\quad\quad\quad\quad|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & \lesssim 
    p^{a + t + s + L_2(K)+ r-\xi + \frac{1}{2}(b + a + s +L_2(K)-4 + \xi)}\times 
    |\beta_{1,1}|^{t + b + a + s +L_2(K)-4 + \xi} 
    \times\\
    & \quad\quad\quad\quad\quad\quad\quad\quad|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
\end{split}
\end{equation*}
Now, observe that 
\begin{align*}
    & a + t + s + L_2(K)+ r-\xi + \frac{1}{2}(b + a + s +L_2(K)-4 + \xi)\ge 
    t + b + a + s +L_2(K)-4 + \xi\quad\quad\quad\Longleftrightarrow\\
    & 2r + a + s + L_2 + 4 \ge 3\xi + b,
\end{align*}
which is true since $b + \xi = r + a + s + L_2, 2\xi \le 4.$

Altogether, the above expression becomes 
\begin{align*}
    & |\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{\frac{|V(H)| + \xi - L_1(K)-4}{4}}\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|\times 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|\\
    & = 
    \Bigg(|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}\Bigg)^{|V(H)| + \xi - L_1(K)-4}\times 
    \Bigg(|\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|^{1/3}\Bigg)^3\\
    & \quad\quad\quad\times 
    \bigg(|\ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|^{1/(L_1(K)-\xi + 1)}\Bigg)^{L_1(K)-\xi + 1}\\
    & \le \max(|\ESW_{\SBM(p,1-p,\beta)}(C_4)|^{1/4}, 
    |\ESW_{\SBM(p,1-p,\beta)}(\Star_2)|^{1/3},
    \ESW_{\SBM(p,1-p,\beta)}(\Star_{L_1(K)-\xi})|^{1/(L_1(K)-\xi + 1)}
    )^{|V(H)|}
\end{align*}

==> kSBM.tex <==
\section{SBM models in which each community appears with constant probability}

